Industrial-Strength Model-Based Testing - State of the Art and Current Challenges

As of today, model-based testing (MBT) is considered as leading-edge technology in industry. We sketch the different MBT variants that - according to our experience - are currently applied in practice, with special emphasis on the avionic, railway and automotive domains. The key factors for successful industrial-scale application of MBT are described, both from a scientific and a managerial point of view. With respect to the former view, we describe the techniques for automated test case, test data and test procedure generation for concurrent reactive real-time systems which are considered as the most important enablers for MBT in practice. With respect to the latter view, our experience with introducing MBT approaches in testing teams are sketched. Finally, the most challenging open scientific problems whose solutions are bound to improve the acceptance and effectiveness of MBT in industry are discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{A. Petrenko, H. Schlingloff (Eds.): Eighth Workshop on\\ Model-Based Testing (MBT 2013)\\
EPTCS 111, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.111.1}{10.4204/EPTCS.111.1}}
\pdfoutput=1

